Turning Silver into Gold: Domain Adaptation with Noisy Labels for Wearable Cardio-Respiratory Fitness Prediction

Deep learning models have shown great promise in various healthcare applications. However, most models are developed and validated on small-scale datasets, as collecting high-quality (gold-standard) labels for health applications is often costly and time-consuming. As a result, these models may suffer from overfitting and not generalize well to unseen data. At the same time, an extensive amount of data with imprecise labels (silver-standard) is starting to be generally available, as collected from inexpensive wearables like accelerometers and electrocardiography sensors. These currently underutilized datasets and labels can be leveraged to produce more accurate clinical models. In this work, we propose UDAMA, a novel model with two key components: Unsupervised Domain Adaptation and Multi-discriminator Adversarial training, which leverage noisy data from source domain (the silver-standard dataset) to improve gold-standard modeling. We validate our framework on the challenging task of predicting lab-measured maximal oxygen consumption (VO$_{2}$max), the benchmark metric of cardio-respiratory fitness, using free-living wearable sensor data from two cohort studies as inputs. Our experiments show that the proposed framework achieves the best performance of corr = 0.665 $\pm$ 0.04, paving the way for accurate fitness estimation at scale.

==> 02_related_work.tex <==
\section{Related Work}

%change provides -->enables
\textbf{VO$_{2}$max estimation.} 
% Wearable technology enables applications like activity trackers and smartwatches to measure resting heart rate (RHR) and physical activity and other biosignals in free-living contexts. By leveraging these devices, various silver-standard methods have emerged for more convenient VO$_{2}$max calculation without maximal exercise testing.
% Moreover, several works utilize deep learning techniques for the VO$_{2}$max estimation task \citep{vo2max_ml,vo2max_ml2}. 
% %\cm{you use citep and citeauthor...i think you need consistency?}\yv{fixed}
% For example, some work \citep{vo2max_ml3_rnn} leverages cardiovascular characteristics from seven recreational cyclists to extract VO$_{2}$max by using a recurrent neural network (RNN). 
% \yv{rewrite the above as following: }
Recently, numerous prediction models have been developed using different testing schemes (submaximal exercise / non-exercise tests) and a variety of machine learning methods~\citep{vo2max_ml,vo2max_ml2} to substitute direct measurements of VO$_{2}$max. Specifically, with the help of modern wearable technology, which can track physical activity, resting heart rate (RHR) and other biosignals, various silver-standard methods have emerged for more convenient VO$_{2}$max calculation without maximal exercise testing~\citep{wearble-vo2max,vo2max-non_2,vo2max-non_1,lack-vali-1,lack-vali-3}.
% For example, random forest is utilized to predict VO$_{2}$max via wearable sensors' activity data~\citep{random_forest_vo2max}.
% % \citeauthor{random_forest_vo2max} validated VO$_{2}$max  prediction through wearable sensors' activity data using random forest shallow learning. 
% However, these studies only focus on small cohorts, still contain estimation noise\cm{what noise}, and do not incorporate the gold-standard VO$_{2}$max estimation data. 
% Therefore, although these prior studies provided promising results, we could further improve fitness prediction performance by learning more general patterns from both silver-standard labeled and gold-standard datasets using deep learning methods. 
% \ds{last sentence is quite direct that early in the paper, tone it down}\yv{fixed}
%Motivated by this, 
% In this work, we apply deep learning methods on both large-scale noisy datasets and gold-standard datasets to improve the fitness prediction task.
%\cm{too weak, link better to the intro and our contributions}\yv{fixed}
However, these silver-standard methods generate imprecise VO$_{2}$max estimates, leading to a degeneration of modeling performance and unreliable prediction. 
Recently, a few works applying machine learning models on gold-standard VO$_{2}$max prediction have been proposed~\citep{Abut-2015}: however
% \cm{cite?},\yv{fixed}
they mainly test on small cohorts, which might lead to poor generalization performance. 
% \cm{this sentence is unclear...what do you want to say?}\yv{fixed}
In this paper, we propose a novel DL method that aims to alleviate the distribution difference between imprecise silver-standard data and gold-standard for better VO$_{2}$max prediction (Results are shown in \S\ref{6}).
% \cm{is this ref in the right format? do you mean to say Section?}\yv{fixed}
% \yv{however, these methods mainly use silvver --> which do not have precise labels, performance poor --> leading to unreliable prediction}
% \yv{only using gold lead poor generalization problem}
% \yv{however, in our paper, we propose a method make imprecise silver datsets more silimar/consistent gold, therefore, our methods can achieve better reliable and promising on gold-standard dataset. }


\textbf{Domain adaptation.} A domain combines the input population with the output following a certain probability distribution~\citep{Kouw-2018}. DA is one of the state-of-the-art solutions~\citep{Hoffman-2017} for learning information from an abundant labeled source domain and applying it to a new and unseen target domain with a different distribution.
% \hj{cite CYCADA and read the abstract to learn how to express DA more correctly. Every claim either by data support or by other papers}. \yv{fixed}
DA trains a feature extractor to learn the shared information across domains so the model can generalize to new settings and thus mitigate the domain shift~\citep{Kouw-2018}.
%yv{change especially -> in particular, time tense}
In particular, adversarial-based DA methods show good performance in domain adaptation tasks~\citep{Mei-2018}. Among these methods, Domain-Adversarial Neural Network (DANN)~\citep{Ganin-2015} first introduced adversarial training to domain adaptation. 
DANN utilizes a shared feature extractor to learn feature embedding and a discriminator to maximize the domain difference. After the convergence of the whole training, for each input, general features are learned while their domain information cannot be discriminated.
% \hj{(i.e., their domain information cannot be discriminated)}.\yv{fixed}
% \hj{after "are" are hard to follow}. \yv{fixed}
Followed by this, Domain Separation Networks (DSN)~\citep{Bousmalis-2016} and Adversarial Discriminative Domain Adaptation (ADDA)~\citep{Tzeng-2017} propose more sophisticated feature extraction methods using both shared and private feature extractors for the task classifier and domain discriminator. Moreover, Dual Adversarial Domain Adaptation (DADA)~\citep{Du-2020} uses two discriminators pit against each other to aid the discriminative training. 
% \hj{is there any work specifically work for helth...}\yv{mentioned in next paragraph}

%yv{present tense }
% Recently,
% the majority of applications of DA mainly focus on medical image segmentation and classification tasks ~\citep{Perone-2018, Mei-2020,Venkataramani-2018}.
% \yv{method weakness --> our method novelty}
However, the aforementioned methods mainly focus on discriminating domains as a coarse binary classification task while neglecting the rich information of the domain distribution. Moreover, the majority of applications of DA mainly focus on medical image segmentation and classification tasks ~\citep{Perone-2018, Mei-2020,Venkataramani-2018}. Therefore, we propose a novel DA framework (\systemname{}) with multi-discriminators to learn the coarse-grained and fine-grained domain information and validate on a VO$_{2}$max prediction task.

% Motivated by these methods and given the unique challenges in sensor-based fitness estimation, we propose a novel framework \systemname{} using DA and pre-training to leverage both large unlabeled data from free-living cohorts and lab-based

% \cm{what is lab based data, you never referred to it this way}
% \cm{weak: from this paragraph it appears you are simply applying existing techniques to CRF data}
% \yv{fixed}

% , we propose a novel framework \systemname{} which incorporates source domain knowledge and apply it to the CRF fitness prediction task. To the best of our knowledge, there is no existing work applying DA or adversarial-based DA on VO$_{2}$max prediction task. \ds{kind of weak point again, I would say: given the unique challenges in sensor-based fitness estimation we propose the use of DA and pre-training to leverage both large unlabeled data from free-living cohorts and lab-based data.} \ds{we don't want to be just another ML application paper ;)} \yv{fixed}



==> 04_Datasets.tex <==
\section{Overall Workflow \& Dataset}
\yv{fill the dataset description in, could put data pre-processing and feature extraction in the Appendix part}

% \subsection{Cohort Selection} 
% Two datasets, Fenland and BBVS, are utilized for experiments and evaluations in our work. The Fenland study provides the silver-standard labels (weak labels), while the BBVS dataset uses the directly maximal exercise test and has gold-standard fitness estimation. Specifically, the Fenland study~\citep{feland} is a prospective population-based cohort study of individuals aged 35-65 that aims to investigate the interaction between environmental and genetic factors in determining obesity, type 2 diabetes, and related metabolic disorders. The study has collected from 12,435 participants around Cambridgeshire in the East of England between 2005 and 2015. After a baseline clinic visit, participants were asked to wear a combined heart rate and movement chest sensor Actiheart for six whole days. 
% The BBVS dataset is a subset of 191 participants from the Fenland study and aims to validate CRF measurements methods for the UKB-CRF test \yv{citep{BBVS}}. During the study, electrocardiography~(Cardiosoft) and an Actiwave CARDIO device~(CamNtech, Papworth, UK) were utilized to collect signals and directly measured VO$_{2}$max. 
% All participants from two datasets provided written informed consent, and the University of Cambridge Ethics Committee approved the study. 

% \subsection{Data extraction} 
% In the Fenland study, VO$_{2}$max was measured through a heart rate-to-work rate linear regression method across several ramped treadmill tests\citep{gonzales2020submaximal}. Participants wore the two standard Electrocardiography (ECG) electrodes Actiheart devices attached to the chest, which measured heart rate and movement recording at 60-second intervals~\citep{actiheart}. The monitoring phase continued for six complete days. During a lab visit, all participants performed a treadmill test to establish their individual response to a submaximal test, informing their VO$_{2}$max (maximum rate of oxygen consumption measured during incremental exercise)~\citep{submax-test}. HR was recorded for 15 minutes, and RHR was calculated as the mean heart rate measured during the last 3 minutes. The RHR is a mix of the RHR mentioned above and the Sleeping HR as recorded by the ECG during the free-living period.

% Participants in the BBVS research were screened using the same standardized techniques used for the UKB-CRF test~\citep{CRF-manual}. Following that, participants did 5 maximal exercise tests to elicit VO$_{2}$max, including a UKB flat test, two UKB ramped tests with varying ramp rates, and a steady-state test (exclusive to the validation study), and another ramped test (for validation only). The tests were done sequentially, with at least 15 minutes of rest between each.


\subsection{Feature Choices} 
% All heart rate data collected during free-living conditions underwent pre-processing for noise filtering~\citep{noise-filter}. If participants had fewer than 72 hours of concurrent wear data (three full days of recording) or inadequate individual calibration data, they were eliminated from the study (treadmill test-based data). Non-wear periods were excluded from the analyses through non-wear detection procedures. This pre-processing algorithm discovered lengthy durations of non-physiological heart rate and extended periods of no movement reported by the device's accelerometer (\textgreater 90 minutes). We used the calculation 1 MET = 71 J/min/kg (3.5 ml O2 min1 kg1) to convert movement intensities into standard metabolic equivalent units (METs). These conversions were then used to classify intensity levels, with behaviors less than 1.5METs classed as sedentary, those between 3 and 6 METs as moderate to vigorous physical activity (MVPA), and those greater than 6METs as vigorous physical activity (VPA). Since time can greatly impact physical activities, we encoded the sensor timestamps using cyclical temporal features \citep{Spathis_self_supervision}. 

% Additionally, given the sensors' high sampling rate (1 sample/minute) after matching the HR and Acceleration modalities, learning patterns from such a lengthy sequence (a week's worth of sensor data contains more than 10,000 timesteps) is unfeasible, even with the most potent recurrent neural networks. Therefore, our models downsampled the sampling rate to 15 minutes and used the first 600 timesteps to represent each participant's feature vector. Then each feature vector with 26 features combing time-series and metadata was put into various deep neural networks. A detailed view of these features is provided in Table~\ref{tab:variables}.

\subsection{Data Preparation } 
% For unsupervised learning and transfer learning, we divided them into two steps procedures: pre-training on the silver-standard dataset and fine-tuning to the dataset with gold standard fitness estimation. For each task, the data preparation details are described as follows. 
 
% The first step explored the pre-training networks on the Fenland dataset. Here, we matched sensor data with lab test results from eligible ones. Then we divided it into training and testing sets, with the training set further split into training and validation datasets (90 - 10$\%$). After splitting the dataset, we normalize the training data by applying min-max scaling on all features(sequence-wise for time-series features \(x_i\)\ and column-wise for meta-features \(m_i\)~\citep{Spathis_self_supervision}. 

% For the second step, to learn the distribution shift and prove the importance of presentation learning from the dataset with noise estimation, we performed different fine-tune strategies on BBVS. We divided the BBVS dataset into train and test sets (80 - 20$\%$) based on five random seeds [42, 12, 123, 1231, 12312] because of the limited sample size after matching the sensor data. A visual representation of these tasks' data splitting can be found in Figure~\ref{task-info}.

%may put the pre-processing the data preparation steps in the Appendix. 



==> 05_experiments.tex <==
% \section{Experiments}\label{experiment}
% % prensest tense instead of past tense
% %change words (validate, quantiy)
% We conduct various qualitative and quantitative evaluations to validate our models on the cardio-respiratory fitness prediction task (\S\ref{5.1}) and compare it with different baselines (\S\ref{5.2}). We then further quantify the impact of incorporating source domain knowledge to \systemname{} (\S\ref{5.3}).
% % \hj{section label is wrong}.\yv{fixed} 
% The overall workflow is depicted in Figure~\ref{fig:workflow}.

% \subsection{Datasets and Training Strategy}\label{5.1}
% % \yv{add clear datasets descriptionxx, label difference(exercise test), same sensor xxx}

% \textbf{Datasets.} The source domain comes from the silver-standard measurement study (Fenland), including 12,425 participants. It contains a combined heart rate and movement signal from chest ECG sensor Actiheart and noisy VO$_{2}$max labels collected from submaximal exercise tests~\citep{feland}. 
% The target domain \(\bm{D_t}\) represents the gold-standard measurement dataset BVS, which is a subset of 191 participants from the Fenland study with directly measured ground-truth VO$_{2}$max~\citep{bvs} during the maximal exercise tests. In the BVS study, participants need to wear a face mask to measure respiratory gas measurements~\citep{Rietjens-2001} to experience exhaustion tests. % for the data collection \ds{awkward sentence}. \yv{fixed}
% Further, movement and heart rate are collected using the Actiheart (CamNtech, Papworth, UK) sensor.
% A detailed description of these two datasets is provided in Appendix~\ref{apd:first}.
% % \hj{I think you did it in Figure 2?}
% % \hj{Missing sth. You want to say: "To utilize these datasets to train \systemname{}, we first?? xxx"?}\yv{fixed}

% \textbf{Training Strategy.} We evaluate \systemname{} on these two datasets by first pre-training a model on the \(\bm{D_s}\) Fenland. 
% % \ds{repetition!}\yv{fixed}
% Second, we develop the adversarial training framework with multi-discriminators on the BVS (\(\bm{D_t}\)), with the help of incorporated prior domain knowledge (i.e., injecting random samples from the source domain). For each domain, feature choices are in Appendix~\ref{apd:first}. 
% % \ds{elaborate here}\yv{fixed}. 
% After the adversarial adaptation, we predict VO$_{2}$max on the held-out test set of BVS using 3-fold cross-validation using \systemname{}. Within each fold, the dataset is split into 70\% training and 30\% testing consisting only of target domain samples.
% % \yv{we first split the dataset and then incorporate the source domain samples..., make sure at least 30\% BVS is used to test the model... }

% % the dataset was split into 66\% of training with \hj{with how many sample? ie. 9,321}, and 34\% of testing samples with  samples consisting only of the original target domain samples.
% % \yv{around 70\% and 30\%}

% % Specifically, we mixed the target domain source\hj{?} BVS dataset, with gold-standard labeled VO$_{2}$max measurements with part of prior knowledge from the Fenland dataset\hj{not a complete sentence in semantic}. Finally, we fine-tuned the pre-trained encoder \hj{throughr three layers MLP?} on the new mixture domain training set and evaluated the predictor performance on the test set using the 3-fold cross-validation using \systemname{}. Within each fold, the dataset was split into 70\% of training \hj{with how many sample? ie. 9,321}, and 30\% of testing samples consisting only of the original target domain samples.

% % \textcolor{red}{or we should put hyper-parameter tuning in the appendix}


% \subsection{Baselines}\label{5.2}
% % \yv{add features and pre-processing? in the appendix}
% % \yv{should the input need to be very detail?use notation or specific fenland/bvs? or general information}
% To verify the effectiveness of our proposed network, we compare the \systemname{} against several baselines:
% % ~\hj{replace all UDAMA with macro command \systemname{}}
% \begin{itemize}
%     \item \textbf{Train from Scratch.} A network with the same structure as the pre-training model utilize wearable data and common biomarkers 
%     % \ds{do we mention the features anywhere? put in appendix if u have time} \yv{fixed}
%     in \(\bm{D_t}\) as input to predict VO$_{2}$max.
%     % \ds{talk about inputs and outputs here} \yv{fixed}
%     % \hj{on gold only right?}
%     \item \textbf{Transfer learning.}  A pre-trained model trained on \(\bm{D_s}\) is reused and fine-tuned on the target domain. 
%     % \ds{just say fine-tuned on the target domain} \yv{fixed}
%     % \hj{what is upstream? you want to say the model trained from scratch?}
%     \item \textbf{Transfer learning with Incorporated Source Domain Knowledge.} Based on the aforementioned transfer learning baseline, we fine-tune the pre-trained model on the combination of \(\bm{D_t}\) and incorporated samples from \(\bm{D_s}\) to predict VO$_{2}$max on \(\bm{D_t}\). 
%     % we inject samples from the source domain directly without using the adversarial training structure. 
%     % \ds{unclear, inputs+outputs pls} \ds{Is this our idea or can we cite?}\yv{our ideas}
%     \item \textbf{Domain Adversarial Neural Networks (DANN)~\citep{Ganin-2015}.} A benchmark domain adaption method which uses adversarial training for binary domain classification. 
    
% \end{itemize}

% \subsection{Effect of Injected Source Domain Samples}\label{5.3}
% % \yv{should we use percentage or numbers of samples?}~\hj{percentage}
% % \hj{I assume we need to discuss why we want to do this. e.g., to examine whether our model is impacted by only specific samples, we further investigate...}
% % To examine \ds{assess the degree in which} \yv{fixed}
% To assess the degree to which the incorporated source domain knowledge impacts our model, we evaluate \systemname{} on different levels of 
% % \yv{how to display these percentage better...}
% samples sizes from ($\bm{D_s}$). As such, we put \{0.1\%, 0.2\%, 0.4\%, 1\%, 2\%, 4\% \} of $\bm{D_s}$,
% % \ds{check notation, is it bm?}\hj{fixed}, 
% which equals to \{1\%, 5\%, 10\%, 30\%, 50\% and 100\%\} of training data of the target domain ($\bm{D_t}$).
% % (equals to 1\%, 5\%, 10\%, 30\%, 50\% and 100\%  of training data of the target domain ($D_t$).
% We set the maximum amount to 100\% because for any larger amount, the model would be trying to predict
% % \cm{predict? unclear what help means here}\yv{fixed}
% the silver data rather than the gold data.
% % \hj{We set the maximum amount of 100\% because larger than that the model is trying to help the silver data rather than the gold data.}
% % \ds{why up to 4\% only?} \hj{equals to 1\%, 2?\%, 50?\%,  to 100\% amount of train data of the target domain} \yv{fixed}
% % \cm{sentence dandling?} \yv{fixed, by deleting sentence: samples from xxxx}
% % samples from the Fenland\Rmnum{2} dataset $D_s$, the testsetwe evaluate the pre-training model, 
% Then, we run the experiments 15 times with different seeds to assess the impact of the injected noisy samples.
% % \ds{impact of what?} \yv{fixed}
% using the average performance on the VO$_{2}$max prediction task. Results are shown in \S\ref{6.3}.
% % \hj{use label and ref}. 


% \subsection{Implementation and Metrics}
% % \yv{add hyper-parameter tuning results in appendix?}\hj{if out paged, yes}
% All network blocks in the framework are trained using Adam with  learning rate being tuned over \{${1e^{-2}}, {1e^{-3}}, {1e^{-4}}, {1e^{-5}}$\}. The dropout rate is tuned over the following ranges \{0.2, 0.3\}. Moreover, we tune the batch size between 8, 16, and 32 based on the efficiency and stability of the training process.
% % \hj{?} \yv{to describe how to tune the variables in the total loss function} 
% To tune the \systemname{} total loss, we conduct a grid search~\{0.01, 0.02, 0.03\} for the $\alpha$ and~\{(0.9, 0.1), (0.8, 0.2), (0.7, 0.3), (0.6, 0.4), (0.5, 0.5)\} for the combination of $\lambda_1$ and $\lambda_2$. We perform early stopping to combat overfitting until the validation loss stops improving after 10 epochs. 
% % \hj{how many steps for early stopping?}\yv{?}

% \textbf{Metrics.} The prediction performance of all models is evaluated based on standard regression evaluation metrics such as the Mean Squared Error (MSE) and Mean Absolute Error (MAE). The coefficient of determination (R$^2$) and the Pearson correlation coefficient (Corr) are also used to evaluate the model performance on the health-related outcome prediction task.





==> 06_results_discussion.tex <==
\section{Results and Discussion}\label{6}
\begin{table*}
  \small
  \caption{\textbf{Evaluation of different methods to predict VO$_{2}$max on the BVS test set.} Each result displays the mean value with standard deviation from three-fold cross-validation. In particular, the results of \systemname{} come from incorporating 5\% amount of BVS samples From Fenland.}
  \begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} llll}
  \toprule
    \textbf{Method} & \textbf{R$^2$} & \textbf{Corr} &  \textbf{MSE} & \textbf{MAE} \\ 
    \midrule
    Train from scratch & -0.096 $\pm$ 0.100 & 0.007 $\pm$ 0.250 & 58.048 $\pm$ 10.061  & 6.336 $\pm$ 0.621  \\ 
    Transfer learning (TF)  & 0.362 $\pm$ 0.036  & 0.647 $\pm$ 0.032 & 31.970 $\pm$  4.184 & 4.552 $\pm$ 0.350
 \\ 
    TF with added samples & 0.288 $\pm$ 0.077   & 0.617 $\pm$ 0.037 & 35.458 $\pm$ 3.920 & 4.679 $\pm$ 0.382  \\ 
    DANN~\citep{Ganin-2015}  & 0.367 $\pm$ 0.048& 0.647 $\pm$ 0.035& 31.734 $\pm$ 4.753  & 4.536 $\pm$ 0.422   \\
    \textbf{UDAMA (ours)} & \textbf{0.508} $\pm$ \textbf{0.096} & \textbf{0.725} $\pm$ \textbf{0.058} &  \textbf{24.912} $\pm$ \textbf{6.794} & \textbf{3.942} $\pm$ \textbf{0.521} \\
    \bottomrule
  \end{tabular*}
  \label{table-results}
  \vspace{-0.1in}
\end{table*}

We present the results of applying \systemname{} on the VO$_{2}$max prediction task and compare it to the baselines (\S\ref{6.1}). Additionally, we discuss the performance related to the domain shift problem (\S\ref{6.2}) and the impact of injected source domain knowledge (\S\ref{6.3}). Furthermore, we conduct the ablation study to verify the effectiveness of our framework's structure (\S\ref{6.4}). Finally, we discuss  model interpretability in \S\ref{6.5}. 


\subsection{VO2max prediction}\label{6.1}
The comparison of the proposed domain adaptation framework and baseline approach for VO$_{2}$max prediction is shown in Table~\ref{table-results}. 
%According to Table~\ref{table-results}, our results show that 
The proposed framework outperforms all baselines for this prediction task and yields the best results among all evaluation metrics. We observe that the correlation (Corr) outperforms the basic transfer learning methods by 12.1\%, the MSE increases by 22.1\%, and R$^2$ improves by 40.3\% compared to the baseline Transfer Learning method. 
% \yv{added stats supports}
Notably, we observe that baseline results also reinforce the importance of our proposed framework. For example, after incorporating source domain samples into basic TF models, R$^2$, Corr, and MSE drop by 20.4\%, 4.6\%, and 10.9\% compared to TF. 
%Given this performance degeneration, 
We attribute this performance degeneration to the fact that the injected samples would not improve the fine-tuning on the target domain and introduce noise due to the distribution mismatch, resulting in negative transfer (i.e., decreasing the TF performance).

% \hj{resulting negative transfer (i.e., decreasing the modeling performance)} \hj{which model?} .\yv{fixed}
% \hj{Same here. Claims need supports from numbers, i.e., 30\% of improvement (from xxx to xxx)}

% \begin{figure}
%     \centering
%     \includegraphics[width=2.5 in]{Images/Fenland_BVS_Distribution.png}
%     \caption{\textbf{Distribution of BVS and Fenland dataset.}}
%     \label{fig:ori-distribution}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=2.5 in]{Images/Domain_shift.png}
%     \caption{\textbf{Distribution of prediction from different methods and the ground-truth BVS.}}
%     \label{fig:distribution-shift}
% \end{figure}

% \begin{figure*}[!t]
% \centering
%   % \centering
%   \subfloat[Uncertainty classifier in TFLM format]{
%   \includegraphics[width=.34\textwidth]{images/deployment/head.pdf}
%   \label{fig:operator_ur2m}
%   }
%   \subfloat[MCU library optimization]{
%     \includegraphics[width=.66\linewidth]{images/memory_saving.pdf}
%   \label{fig:memory_sram}
%   }
%   \caption{Deployment stagy. (a) Uncertainty deployment on MCU based on multiple operators to calculated uncertainty and classification result. (b) MCU library space before optimization (top) and after optimization (bottom).
%   % \dm{what is the optimization?}\hj{fixed in Section 5.4}
%   }
% \label{fig:implementation}
% \end{figure*}


\begin{figure*}[]
  \centering 
  % \subfloat[]{
  \subfigure[]{
  \begin{minipage}[]{0.5\textwidth}
  \centering
  \includegraphics[width=2.5 in]{Images/Fenland_BVS_Distribution.png} 
  \end{minipage}
  \label{fig:ori-distribution}
  }
  \subfigure[]{
  % \subfloat[]{
  \begin{minipage}[]{0.4\textwidth}
  \centering
  \includegraphics[width=2.5 in]{Images/Domain_shift.png} 
  \end{minipage}
  \label{fig:distribution-shift}
  }
  \caption{\textbf{\systemname{} mitigates distribution shifts.} Visualization of VO$_{2}$max distribution. \textbf{(a)} The distribution of BVS and Fenland dataset. \textbf{(b)} Distribution of prediction from different methods and the ground-truth BVS. 
%   \yv{working on replotting the figure}
%   \hj{replot make them wide and trim margins}
  }
  \label{fig:distribution}
   \vspace{-0.2in}
\end{figure*} 

\subsection{Domain shift}\label{6.2}
% \yv{add f-divergences to calculate the distance between two distribution), mean of distribution}
% \hj{why you want to do this?}\yv{fixed}
% Domain shift will decrease the model efficiency and accuracy when a model is trained from one dataset to another. 
% \hj{put these summary words into last paragraph. Here instead to say "we examine whether \systemname{} can effectively xxx"} \yv{fixed}
We examined whether \systemname{} can effectively solve the domain shift problem. We observe that our proposed domain adaptation framework can effectively alleviate the problem. Figure~\ref{fig:ori-distribution} shows that the \(\bm{D_s}\) dataset (i.e., Fenland) shares a different VO$_{2}$max underlying distribution compared to \(\bm{D_t}\) BVS. Our results in Figure~\ref{fig:distribution-shift} show that our framework learns the small dataset distribution during the adaptation phase and achieves promising results compared with other methods. To examine the distance between domains, we use the Hellinger
% \cm{Hellinger maybe? } \yv{fixed, Heelingence -->Hellinger}
Distance (HD) to calculate the similarity of distributions between the prediction and the ground truth. Specifically, our framework's prediction of fitness level lies in the same range as the ground truth, where the mean of the \systemname{} is 32.13\si{\milli\liter\per\kilogram\per\min}, and the mean of BVS is 32.53\si{\milli\liter\per\kilogram\per\min}.
% \ds{in what units is this measured?}. 
Besides, distribution ties close compared to baseline methods, where the normalized HD for \systemname{} is 0.143, and HD for TF is 0.215. These results indicate that our framework can effectively alleviate the distribution shift problem of the VO$_{2}$max prediction task. As a result, we reduce the difference between noisy silver-standard data and gold-standard data and improve the gold-standard model performance. 
% \ds{add final sentence why this distance experiment is important for our method} \yv{fixed}
% \hj{add numbers}. \yv{fixed} 

\begin{figure}
    \centering
    \includegraphics[width=2.5 in]{Images/trend0831.png}
    \caption{\textbf{Impact of injected source domain samples. }}
    \label{fig:scale}
    \vspace{-0.1in}
\end{figure}



\subsection{Impact of Injected Knowledge from Source Domain}\label{6.3}
Figure~\ref{fig:scale} shows the average performance of adding the different scales of injected source domain samples to the target domain.
Each boxplot shows the average MSE results of 15 different runs with added random samples. 
% \yv{how can we describe this better?}
As shown in Figure~\ref{fig:scale}, our method performs better than the baseline methods with added samples in all cases, even after adding 100\% of noisy samples of $\bm{D_t}$ from $\bm{D_s}$.
% even add 100\% amount of \(\bm{D_t}\) training set (4\% from the \(\bm{D_s}\))\cm{last part unclear}.\yv{rephrase to: even adding 100\% amount noisy samples of $\bm{D_t}$ from $\bm{D_s}$?}
Specifically, we observe that by only adding 0.2\% from the source domain, which equals 5\% of \(\bm{D_t}\),
% \cm{say also the percentage on the target domain?}\yv{fixed} 
it achieves the best results and showcases the most positive transfer. We postulate that this is because 
%this result originates from 
the small injected samples have a random distribution,
% \ds{you mean normal dist? be specific here}, \yv{delete general}
This is not similar to either the source or target domain, as shown in Figure~\ref{fig:added-sample-distribution}. 
% Therefore, this randomness helps enhance the model's performance\hj{a little bit weak. extend a little bit}.\yv{how can we describe this?}\hj{I guess we need to focus on either DA or this randomness. If it is the first one, simply comment it as it is not a claim or contribution.}\yv{fixed}

% On the other hand, when adding more samples from the source domain, we observe the negative transfer because of incorporating more noisy distribution knowledge\hj{why? data support?}. As shown in the distribution plot, when adding 5\% percent of source domain data, the performance will decrease by xxx. \yv{add percentage}Thus, the pre-trained encoder would tend to learn the source domain data points better instead of focusing on improving the target domain prediction task \hj{i.e., in [distrubiton plot] shows xxx}.   
\begin{figure}
    \centering
    \vspace*{3.5ex}\includegraphics[width=2.5 in]{Images/random-sample-distribution.png}
    \caption{\textbf{Distribution of injected source domain samples.}}
    \label{fig:added-sample-distribution}
    \vspace{-0.1in}
\end{figure}


\begin{table*}
  \centering 
  \small 
  \caption{\textbf{Ablation study by removing one of the discriminators.
%   Evaluation of different discriminators.}\hj{Ablation study by removing one of the discriminators;add MAE}\yv{fixed}
   }}
%   \resizebox{1\columnwidth}{!}{
  \begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} llll}
  \toprule
    \textbf{Discriminator} & \textbf{R$^2$} & \textbf{Corr} & \textbf{MSE} & \textbf{MAE} \\
    \midrule
    Coarse-grained & 0.441 $\pm$ 0.065 & 0.692 $\pm$ 0.038 & 28.132 $\pm$ 5.411 & 4.263 $\pm$ 0.423 \\ 
    Fine-grained  & 0.467 $\pm$ 0.105 & 0.713 $\pm$ 0.054 & 26.938 $\pm$ 7.422 & 4.137 $\pm$ 0.497 \\ 
    \textbf{UDAMA (ours)} & \textbf{0.508 $\pm$ 0.096} & \textbf{0.725 $\pm$ 0.058} &  \textbf{24.912 $\pm$ 6.794} & \textbf{3.942 $\pm$ 0.521} \\
    \bottomrule
  \end{tabular*}

  \label{table:ablation study} 
\end{table*}

\begin{figure*}[]
  \centering 
  % \subfloat[]{
  \subfigure[]{
  \begin{minipage}[]{0.45\textwidth}
      \centering
  \includegraphics[width=2.5 in]{Images/RAM_tf_0831.png} 
  \end{minipage}
  \label{fig:ram-tf}
  }
  % \subfloat[]{
  \subfigure[]{
  \begin{minipage}[]{0.45\textwidth}
      \centering
  \includegraphics[width=2.5 in]{Images/RAM_da_0831.png} 
  \end{minipage}
  \label{fig:ram-da}
  }
  \caption{\textbf{Regression activation mapping (RAM).}
%   \hj{again, why do this, link each sentences. and add a summary}
  Visualizing important regions in timestamps using RAM. The color of each dot represents the importance that the model is looking at while predicting the VO$_{2}$max. The number in the title indicates the MSE error of prediction. \textbf{(a)} RAM output for transfer learning.
  \textbf{(b)} RAM output for \systemname.
%   \hj{We did not use RMSE; normalize bar}\yv{fixd}
  }
  \label{fig:ram}
  \vspace{-0.3in}
\end{figure*}  
%Ablation study -- discuss which discriminators should add and what's the performance

\subsection{Ablation Study} \label{6.4}
Our framework comprises two joint discriminators, and hence we perform an ablation study to understand each discriminator's effect.
Based on the observation that incorporating 5\% amount of BVS from the \(\bm{D_t}\) Fenland dataset
% \cm{it's 5 percent of the target domain right?}\yv{fixed} 
achieves the best transfer, we train different discriminators under this setting. We observe that a single discriminator (coarse-grained or fine-grained) exhibits more competitive performance than the baseline TF methods, as shown in Table~\ref{table:ablation study}. Specifically, the fine-grained discriminator alone significantly outperforms the baseline results: +15.1\% TF (based on MSE). This indicates that utilizing more fine-grained distribution domain labels helps the adversarial training framework learn the cross-domain information and improves the main prediction task. 

\subsection{Interpretability}\label{6.5}

% \hj{why you want to do this? e.g., to understand why our DA framework can effectively ... we further examine the salience map of our ...}
To understand the effectiveness of \systemname{}, we further examine the saliency 
% \cm{saliency map i think}\yv{fixed}
map to interpret predictions on the datapoint level. Motivated by recent works~\citep{cam-timeseries,RAM,cam}, we employ the regression activation mapping (RAM) framework to visualize which timestamps were relevant to the respective VO$_{2}$max value.
% Class activation maps~\citep{cam} is a simple yet robust technique used in image classification tasks to visualize which regions in the image were relevant to each respective class. \hj{link between these two sentences} Our work aims to visualize relevant timesteps in the raw data for VO$_{2}$max prediction. Motivated by \citeauthor{cam-timeseries,RAM}, we employ the regression activation mapping (RAM) framework for time-series data.
Figure~\ref{fig:ram} shows the RAM 
% \cm{do you define ram before?}\yv{yes}
output for the same participant using the transfer-learning method and \systemname{} on the raw accelerometer data. Notably, for \systemname{}, we observe that the regions in~\ref{fig:ram-da} that contribute to estimations are distinct. \systemname{} can capture the temporal dynamics of the feature, manifested by the higher score in the later section of the week, which seem to help the model predict the fitness score more accurately. Instead, TF rates every timestamp equally, as shown in Figure~\ref{fig:ram-tf}, which is not meaningful and can manifest in low accuracy. This demonstrates that \systemname{} has better interpretability and robustness than TF. 
% \ds{i tried to fix this section}


% As shown in the figure, The result demonstrates that \systemname{} shows better interpretability than the transfer learning method, which simply considers every timestamp as equally important. Apart from lower error, \systemname{} captures the temporal dynamics of the specific feature (wearable acceleration), manifested by the higher score in the later section of the week which seem to help the model predict the fitness score more accurately. 
% \hj{As such, a .... add a sum of this paragraph}

